Robust Medical Instrument Segmentation Challenge 2019

Intraoperative tracking of laparoscopic instruments is often a prerequisite for computer and robotic-assisted interventions. While numerous methods for detecting, segmenting and tracking of medical instruments based on endoscopic video images have been proposed in the literature, key limitations remain to be addressed: Firstly, robustness, that is, the reliable performance of state-of-the-art methods when run on challenging images (e.g. in the presence of blood, smoke or motion artifacts). Secondly, generalization; algorithms trained for a specific intervention in a specific hospital should generalize to other interventions or institutions. In an effort to promote solutions for these limitations, we organized the Robust Medical Instrument Segmentation (ROBUST-MIS) challenge as an international benchmarking competition with a specific focus on the robustness and generalization capabilities of algorithms. For the first time in the field of endoscopic image processing, our challenge included a task on binary segmentation and also addressed multi-instance detection and segmentation. The challenge was based on a surgical data set comprising 10,040 annotated images acquired from a total of 30 surgical procedures from three different types of surgery. The validation of the competing methods for the three tasks (binary segmentation, multi-instance detection and multi-instance segmentation) was performed in three different stages with an increasing domain gap between the training and the test data. The results confirm the initial hypothesis, namely that algorithm performance degrades with an increasing domain gap. While the average detection and segmentation quality of the best-performing algorithms is high, future research should concentrate on detection and segmentation of small, crossing, moving and transparent instrument(s) (parts).

==> rankingsS1S2.tex <==
\subsection{Rankings for stage 1}
\label{app:ranking-s1}
\subsubsection{Binary segmentation}
As described in sec.~\ref{sec:rankings}, an accuracy and a robustness ranking were computed for both metrics, the DSC and the NSD. This results in four rankings for the binary segmentation task. 

\begin{table}[h]
    \caption{Binary segmentation: Accuracy ranking for the DSC in stage 1 of the challenge.}
    \label{tab:s1-bs-dsc-accuracy}
    \renewcommand{\arraystretch}{1.3}
    \centering
    \begin{tabular}{l c c}
    \hline
        \textbf{Team identifier} & \textbf{Prop. Sign.} & \textbf{Rank}\\ \hline
        \textbf{Isensee} & \textbf{0.9} & \textbf{1} \\ 
        haoyun & 0.7 & 2 \\ 
        CASIA\_SRL & 0.7 & 2\\ 
        Caresyntax & 0.5 & 4 \\ 
        Uniandes & 0.5 & 4 \\ 
        Prometheus & 0.4 & 6 \\ 
        SQUASH & 0.3 & 7 \\ 
        www & 0.2 & 8 \\ 
        VIE & 0.1 & 9 \\ 
        NCT & 0.0 & 10 \\ \hline
    \end{tabular}
\end{table}

\begin{table}[h]
    \caption{Binary segmentation: Robustness ranking for the DSC in stage 1 of the challenge.}
    \label{tab:s1-bs-dsc-robust}
    \renewcommand{\arraystretch}{1.3}
    \centering
    \begin{tabular}{l c c}
    \hline
        \textbf{Team identifier} & \textbf{Aggr. DSC Value} & \textbf{Rank}\\ \hline
        \textbf{Isensee} & \textbf{0.759} & \textbf{1 }\\ 
        Uniandes & 0.715 & 2 \\ 
        CASIA\_SRL & 0.697 & 3\\ 
        Caresyntax & 0.689 & 4 \\ 
        www & 0.679 & 5 \\ 
        haoyun & 0.643 & 6 \\ 
        SQUASH & 0.547 & 7 \\ 
        Prometheus & 0.488 & 8 \\ 
        VIE & 0.301 & 9 \\ 
        NCT & 0.043 & 10 \\ \hline
    \end{tabular}
\end{table}

\begin{table}[h]
    \caption{Binary segmentation: Accuracy ranking for the NSD in stage 1 of the challenge.}
    \label{tab:s1-bs-nsd-accuracy}
    \renewcommand{\arraystretch}{1.3}
    \centering
    \begin{tabular}{l c c}
    \hline
        \textbf{Team identifier} & \textbf{Prop. Sign.} & \textbf{Rank}\\ \hline
        \textbf{Isensee} & \textbf{0.9} & \textbf{1} \\ 
        haoyun & 0.6 & 2 \\ 
        CASIA\_SRL & 0.6 & 2\\ 
        Uniandes & 0.6 & 2 \\ 
        Caresyntax & 0.4 & 5 \\ 
        www & 0.3 & 6 \\ 
        Prometheus & 0.3 & 6 \\ 
        SQUASH & 0.2 & 8 \\ 
        VIE & 0.1 & 9 \\ 
        NCT & 0.0 & 10 \\ \hline
    \end{tabular}
\end{table}

\begin{table}[h]
    \caption{Binary segmentation: Robustness ranking for the NSD in stage 1 of the challenge.}
    \label{tab:s1-bs-nsd-robust}
    \renewcommand{\arraystretch}{1.3}
    \centering
    \begin{tabular}{l c c}
    \hline
        \textbf{Team identifier} & \textbf{Aggr. NSD Value} & \textbf{Rank}\\ \hline
        \textbf{Isensee} & \textbf{0.842} & \textbf{1} \\ 
        www & 0.796 & 2 \\ 
        Uniandes & 0.789 & 3\\ 
        CASIA\_SRL & 0.771 & 4 \\ 
        haoyun & 0.743 & 5 \\ 
        Caresyntax & 0.741 & 6 \\ 
        SQUASH & 0.691 & 7 \\ 
        Prometheus & 0.625 & 8 \\ 
        VIE & 0.256 & 9 \\ 
        NCT & 0.090 & 10 \\ \hline
    \end{tabular}
\end{table}

\subsubsection{Multiple instance detection}
\begin{table}[h]
    \caption{Multiple instance detection: Ranking for the mAP in stage 1 of the challenge.}
    \label{tab:s1-mid-map}
    \renewcommand{\arraystretch}{1.3}
    \centering
    \begin{tabular}{l c c}
    \hline
        \textbf{Team identifier} & \textbf{Aggr. mAP Value} & \textbf{Rank}\\ \hline
        \textbf{Isensee} & \textbf{1.000} & \textbf{1} \\ 
        \textbf{Uniandes} & \textbf{1.000} & \textbf{1} \\ 
        SQUASH & 0.967 & 3\\ 
        Caresyntax & 0.944 & 4 \\ 
        www & 0.900 & 5 \\ 
        VIE & 0.75 & 6 \\ \hline
    \end{tabular}
\end{table}

\subsubsection{Multiple instance segmentation}
\begin{table}[h]
    \caption{Multiple instance segmentation: Accuracy ranking for the MI\_DSC in stage 1 of the challenge.}
    \label{tab:s1-mis-dsc-accuracy}
    \renewcommand{\arraystretch}{1.3}
    \centering
    \begin{tabular}{l c c}
    \hline
        \textbf{Team identifier} & \textbf{Prop. Sign.} & \textbf{Rank}\\ \hline
        \textbf{Isensee} & \textbf{0.875} & \textbf{1} \\ 
        Uniandes & 0.750 & 2 \\ 
        Caresyntax & 0.625 & 3\\ 
        SQUASH & 0.375 & 4 \\ 
        www & 0.375 & 4 \\ 
        CASIA\_SRL & 0.125 & 6 \\ 
        VIE & 0.125 & 6 \\ 
        Prometheus & 0.000 & 8 \\  \hline
    \end{tabular}
\end{table}

\begin{table}[h]
    \caption{Multiple instance segmentation: Robustness ranking for the MI\_DSC in stage 1 of the challenge.}
    \label{tab:s1-mis-dsc-robust}
    \renewcommand{\arraystretch}{1.3}
    \centering
    \begin{tabular}{l c c}
    \hline
        \textbf{Team identifier} & \textbf{Aggr. MI\_DSC Value} & \textbf{Rank}\\ \hline
        \textbf{Uniandes} & \textbf{0.398} & \textbf{1 }\\ 
        www & 0.365 & 2 \\ 
        Caresyntax & 0.325 & 3\\ 
        Isensee & 0.322 & 4 \\ 
        SQUASH & 0.319 & 5 \\ 
        CASIA\_SRL & 0.244 & 6 \\ 
        VIE & 0.161 & 6 \\ 
        Prometheus & 0.102 & 6 \\ \hline
    \end{tabular}
\end{table}

\begin{table}[h]
    \caption{Multiple instance segmentation: Accuracy ranking for the MI\_NSD in stage 1 of the challenge.}
    \label{tab:s1-mis-nsd-accuracy}
    \renewcommand{\arraystretch}{1.3}
    \centering
    \begin{tabular}{l c c}
    \hline
        \textbf{Team identifier} & \textbf{Prop. Sign.} & \textbf{Rank}\\ \hline
        \textbf{Uniandes} & \textbf{0.875} & \textbf{1} \\ 
        Caresyntax & 0.625 & 2 \\ 
        Isensee & 0.500 & 3\\ 
        www & 0.500 & 3 \\ 
        SQUASH & 0.375 & 5 \\ 
        CASIA\_SRL & 0.125 & 6 \\ 
        VIE & 0.125 & 6 \\ 
        Prometheus & 0.000 & 8 \\  \hline
    \end{tabular}
\end{table}

\begin{table}[h]
    \caption{Multiple instance segmentation: Robustness ranking for the MI\_NSD in stage 1 of the challenge.}
    \label{tab:1-mis-nsd-robust}
    \renewcommand{\arraystretch}{1.3}
    \centering
    \begin{tabular}{l c c}
    \hline
        \textbf{Team identifier} & \textbf{Aggr. MI\_NSD Value} & \textbf{Rank}\\ \hline
        \textbf{Uniandes} & \textbf{0.474} & \textbf{1} \\ 
        www & 0.407 & 2 \\ 
        SQUASH & 0.383 & 3\\ 
        Caresyntax & 0.378 & 4 \\ 
        Isensee & 0.346 & 5 \\ 
        CASIA\_SRL & 0.328 & 6 \\ 
        VIE & 0.223 & 7 \\ 
        Prometheus & 0.194 & 8 \\  \hline
    \end{tabular}
\end{table}

\subsection{Rankings for stage 2}
\label{app:ranking-s2}
